An Undetectable Watermark for Generative Image Models

We present the first undetectable watermarking scheme for generative image models. Undetectability ensures that no efficient adversary can distinguish between watermarked and un-watermarked images, even after making many adaptive queries. In particular, an undetectable watermark does not degrade image quality under any efficiently computable metric. Our scheme works by selecting the initial latents of a diffusion model using a pseudorandom error-correcting code (Christ and Gunn, 2024), a strategy which guarantees undetectability and robustness. We experimentally demonstrate that our watermarks are quality-preserving and robust using Stable Diffusion 2.1. Our experiments verify that, in contrast to every prior scheme we tested, our watermark does not degrade image quality. Our experiments also demonstrate robustness: existing watermark removal attacks fail to remove our watermark from images without significantly degrading the quality of the images. Finally, we find that we can robustly encode 512 bits in our watermark, and up to 2500 bits when the images are not subjected to watermark removal attacks. Our code is available at https://github.com/XuandongZhao/PRC-Watermark.

==> archive.tex <==
\section{Introduction}
As AI-generated content grows increasingly realistic, so does the threat of AI-generated misinformation.
Already AI-generated images appeared online in attempts to influence politics (\cite{Mos23}).
Watermarking has the potential to mitigate this issue: If AI providers embed watermarks in generated content, then the content can be flagged using the watermarking key.
However, despite an abundance of watermarking schemes in the literature, adoption has remained limited (\cite{SB23}).
There are at least a few potential explanations for this.
% For instance:
% \begin{itemize}
%     \item OpenAI includes a \emph{metadata} watermark in images generated by ChatGPT and DALL$\cdot$E 3. However, \href{https://web.archive.org/web/20240917123743/https://help.openai.com/en/articles/8912793-c2pa-in-dall-e-3#:~:text=It%20can%20easily%20be%20removed%20either%20accidentally%20or%20intentionally.%20For%20example%2C%20most%20social%20media%20platforms%20today%20remove%20metadata%20from%20uploaded%20images%2C%20and%20actions%20like%20taking%20a%20screenshot%20can%20also%20remove%20it.}{as explained by OpenAI}, metadata watermarks ``can easily be removed either accidentally or intentionally. For example, most social media platforms today remove metadata from uploaded images, and actions like taking a screenshot can also remove it.''
%     \item Google DeepMind launched a watermarking tool called \href{https://deepmind.google/technologies/synthid/}{SynthID} for various kinds of media, but it does not appear to be used by default. We generated images using Gemini, and none of them were detected by \href{https://cloud.google.com/vertex-ai/generative-ai/docs/samples/generativeaionvertexai-imagen-verify-image-watermark}{their publicly-available algorithm}.
%     \item Meta introduced Stable Signature for open-sourced models, but does not appear to use it for Meta AI.
% \end{itemize}
% \sam{TODO cite WSJ article etc.}

% Why is adoption of real watermarking schemes so limited?
% Why might this be the case?
% There are at least a few obvious reasons to explain why watermarks are not widely used in industry.

First, clients are often willing to pay a premium for un-watermarked content.
For instance, a student using ChatGPT to write an essay for a class would find a watermark problematic.
Any company implementing a watermark could therefore put itself at a competitive disadvantage.

Second, existing watermarking schemes do not come with powerful guarantees about the quality, because they noticeably alter the distribution of generated content.
Some schemes guarantee quality preservation for any \emph{single} generation, but introduce correlations across generations.\footnote{One scheme with this guarantee is to fix the randomness of the sampling algorithm, so that the model can only generate one unique response for each prompt.}
While this might be acceptable for small models, it is questionable whether anyone would be willing to introduce such a watermark for a model \href{https://www.wired.com/story/openai-ceo-sam-altman-the-age-of-giant-ai-models-is-already-over/}{that cost over \$100 million just to train}.
Given the vast effort put into optimizing models, it is probable that any observable change in distribution is unacceptable.

Undetectability addresses both of these issues.
For an undetectable watermark, it is computationally infeasible for anyone who doesn't hold the detection key to distinguish generations with the watermark from generations without --- even if one is allowed to make many adaptive queries.
Therefore one can confidently use an undetectable watermark without any concern that the quality might degrade.
And if the detection key is kept sufficiently private, then the competitive disadvantage to using the watermark can be minimized.
One might distribute the detection key only to mass distributors of information (like Meta and X), so that broad dissemination of AI-generated misinformation can be filtered without interfering in users' personal affairs.



% \section*{To do}
% \begin{enumerate}
%     \item Test embedding attack on all schemes
%     \item Test the quality of all schemes
%     \item Try other values of $\texttt{var}$?
%     \item Show the entropy degradation under Gaussian shading
% \end{enumerate}

% \section*{Outline / Organization}
% This section is temporary, just to keep track of what we want to include.

\paragraph{Experiments.}
What PRC parameters should we use? I propose these:
\begin{itemize}
    \item Default:
    \begin{itemize}
        \item $t = 3$
        \item $\text{FPR} = 10^{-9}$
        \item $\text{message\_length} = 512$
        \item $\text{variance} = 1.5$
    \end{itemize}
    \item Max robustness
    \begin{itemize}
        \item $t = 3$
        \item $\text{FPR} = 10^{-2}$
        \item $\text{message\_length} = 0$
        \item $\text{variance} = 1.5$
    \end{itemize}
    \item Max message length
    \begin{itemize}
        \item $t = 4$
        \item $\text{FPR} = 10^{-21}$
        \item $\text{message\_length} = 3000$
        \item $\text{variance} = 0.1$
    \end{itemize}
    \item Max security
    \begin{itemize}
        \item $t = 7$
        \item $\text{FPR} = 10^{-3}$
        \item $\text{message\_length} = 128$
        \item $\text{variance} = 0.1$
        \item $\text{noise\_rate} = 0.08$
        \item $g = 0$
    \end{itemize}
\end{itemize}


% We present the first undetectable watermarking scheme for generative image models.
% We experimentally demonstrate that our watermark does not deteriorate the quality of generated images, in contrast to every prior scheme we tested.
% Our watermark is also robust: existing watermark removal attacks fail to remove the watermark from images without significantly degrading the quality of the image.
% % Furthermore, existing watermark removal attacks fail to remove our watermark from images without significantly degrading the quality of the image.
% Our scheme works by selecting the latents using a pseudorandom error-correcting code (Christ and Gunn, 2024).
% In addition to guaranteeing undetectability and robustness, this technique enables our watermarks to reliably encode up to 2500 bits of information.
% Our experiments use Stable Diffusion 2.1.

% Our watermark is also robust: existing watermark removal attacks fail to remove the watermark from images without significantly degrading the quality of the image.
% We experimentally demonstrate that our watermark does not deteriorate the quality of generated images, in contrast to \emph{every prior scheme} we tested.
% Our watermark is also robust: existing watermark removal attacks fail to remove the watermark from images without significantly degrading the quality of the image.
% In addition to guaranteeing undetectability and robustness, our technique enables our watermarks to reliably encode up to 2500 bits of information.
% Our experiments use Stable Diffusion 2.1.

\section{Introduction} \label{section:intro}
As AI-generated content grows increasingly realistic, so does the threat of AI-generated disinformation.
AI-generated images have already appeared online in attempts to influence politics \citep{Mos23}.
Watermarking has the potential to mitigate this issue: if AI providers embed watermarks in generated content, then that content can be flagged using the watermarking key.
Recognizing this, governments have begun putting pressure on companies to implement watermarks \citep{Bid23,CSL24,EU24}.

% There are at least a few potential explanations for this.

% First, some clients are willing to pay a premium for un-watermarked content.
% For instance, a student using generative AI for class might find a watermark \textcolor{red}{problematic}.
% Any company implementing a watermark could therefore put itself at a competitive disadvantage. \xuandong{I don't know why this premium issue can be addressed by PRC watermark}

However, despite an abundance of available watermarking schemes in the literature, adoption has remained limited \citep{SB23}.
This is largely because watermarking schemes often degrade the quality of generated content. \sam{We can't really say this confidently. Many people claim that the other issue we describe is the main issue}
While some methods ensure that individual responses remain unchanged, they can introduce correlations across multiple outputs.\footnote{One scheme with this guarantee is to fix the randomness of the sampling algorithm, so that the model can only generate one unique response for each prompt.}
Such quality compromises, though tolerable for small-scale models, become unacceptable for high-performance models, which often cost millions of dollars to train~\citep{Wired2023}. Thus any company implementing a watermark could therefore put itself at a competitive disadvantage.

\paragraph{Undetectable watermarks.}
To address these issues, undetectable watermarks offer a promising alternative.
For an undetectable watermark \citep{CGZ24}, it is computationally infeasible for anyone who doesn't hold the detection key to distinguish generations with the watermark from generations without --- even if one is allowed to make many adaptive queries.
Crucially, an undetectable watermark provably preserves quality under any efficiently-computable metric, including quality metrics that are measured across many generations (such as FID \citep{heusel2017gans} and Inception Score \citep{salimans2016improved} for images).
As a result, creators can confidently apply these watermarks without sacrificing content quality, and companies can strategically share the detection keys with large platforms (e.g., Meta and X) to prevent the spread of AI-generated misinformation without restricting everyday users.

% Therefore one can confidently use an undetectable watermark without any concern that the quality might degrade.
% And if the detection key is kept sufficiently private, then the competitive disadvantage to using the watermark can be minimized:
% one can give the detection key only to mass distributors of information (like Meta and X), so that broad dissemination of AI-generated misinformation can be filtered without interfering in users' personal affairs.

% Our scheme is based on the framework for watermarking generative image models introduced by \cite{WKGG23}.

% The key component of our scheme is the application of a pseudorandom error-correcting code (PRC) \citep{CG24}, which encodes the initial latent noise of the LDMs.  This scheme requires no additional training or fine-tuning and can be seamlessly integrated into existing diffusion model APIs. 
% At a high level, a PRC allows us to embed a \emph{cryptographically pseudorandom pattern that is robustly distributed across the entire latent space}.
% We therefore refer to our scheme as the \textbf{PRC watermark} in this work.
